Data Valuation Without Training of a Model

Many recent works on understanding deep learning try to quantify how much individual data instances influence the optimization and generalization of a model. Such attempts reveal characteristics and importance of individual instances, which may provide useful information in diagnosing and improving deep learning. However, most of the existing works on data valuation require actual training of a model, which often demands high-computational cost. In this paper, we provide a training-free data valuation score, called complexity-gap score, which is a data-centric score to quantify the influence of individual instances in generalization of two-layer overparameterized neural networks. The proposed score can quantify irregularity of the instances and measure how much each data instance contributes in the total movement of the network parameters during training. We theoretically analyze and empirically demonstrate the effectiveness of the complexity-gap score in finding `irregular or mislabeled' data instances, and also provide applications of the score in analyzing datasets and diagnosing training dynamics. Our code is publicly available at https://github.com/JJchy/CG_score

==> ICLR2023_CGscore (CameraReady)/fig/dynamic_exp/dynamic_exp.tex <==
\begin{figure*}[!tb]
\centering
	\subfloat[Loss mean \label{fig:dynamic_loss}]{\includegraphics[width=0.33\linewidth]{fig/dynamic_exp/dynamics_loss.png}}
    \subfloat[Accuracy     \label{fig:dynamic_acc}]{\includegraphics[width=0.33\linewidth]{fig/dynamic_exp/dynamics_acc.png}}
    \subfloat[Kernel velocity  \label{fig:dynamic_ntkv}]{\includegraphics[width=0.33\linewidth]{fig/dynamic_exp/dynamic_ntk_velo.png}}
    \caption{Training dynamics measured for each subset of CIFAR-10 examples, grouped by the CG-score. The line color varies over groups, where the blue (red) lines include  low-scoring (high-scoring) examples, respectively. 
    (a) and (b)  Mean loss and accuracy for subgroups of CIFAR-10 data, sorted by the CG-score, trained on ResNet18. The mean loss and accuracy converge slowly for high-scoring groups (red lines).    (c) Kernel velocity of CIFAR-10 examples grouped by the CG-score. The Kernel evolves with a higher velocity for high-scoring groups throughout the training. 
    }
    \label{fig:dynamic_exp}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/gaussian_exp/gaussian_exp.tex <==
\begin{figure*}[!tb]
\centering
	\subfloat[Heat map of $(\rmH^\infty)^{-1}_{n-1}$  \label{fig:gaussian_heatgraph}]{\includegraphics[width=0.28\linewidth]{fig/gaussian_exp/heat_graph_200.png}}
    \subfloat[CG-score (clean) \label{fig:scatter_normal}]{\includegraphics[width=0.28\linewidth]{fig/gaussian_exp/scatter_vi_normal.png}}
% \hfill
    \subfloat[CG-score (10\% label noise) \label{fig:scatter_noise}]{\includegraphics[width=0.42\linewidth]{fig/gaussian_exp/scatter_vi_noise.png}}
    \caption{(a) Heat map of $(\rmH^\infty)^{-1}_{n-1}$ for 200 indices. We plot 200 indices only for clear visualization. (b) Scatter graph of CG-Score for two groups of samples from 3000-D Gaussian distributions having the same mean except the first dimension, where class 1 has mean +1 (red) and class 2 has mean -1 (blue).
Samples near the boundary $(x_1=0)$ tend to have higher CG-score. 
    (c) Same plot as (b) with 10\% label noise. Samples with label noise (marked by plus symbol) tend to have higher CG-score. }
    \label{fig:gaussian_exp}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/noise_exp/noise_detection.tex <==
\begin{figure*}[!tb]
\centering
      \subfloat[Density of CG-score for clean vs. label-noise \label{fig:noise_dist1}]{{\includegraphics[width=0.24 \linewidth]{fig/noise_exp/FMNIST_hist.png}}  
     {\includegraphics[width=0.24 \linewidth]{fig/noise_exp/CIFAR100_hist.png}}}
     \subfloat[Fraction of detected label noise \label{fig:noise_det1}]{{\includegraphics[width=0.24 \linewidth]{fig/noise_exp/FMNIST_detection.png}}
     {\includegraphics[width=0.24 \linewidth]{fig/noise_exp/CIFAR100_detection.png}}}   
    \\ \caption{
    (a) Density of CG-score for clean (80\%) vs. label-noise (20\%) examples. Examples with label noise tend to have higher CG-score.  For FMNIST (left) dataset, the CG-score histograms betwen clean and label-noise groups are better separated than those for CIFAR-100 (right). % dataset, the two histograms have some overlaps. For all the datasets, examples with label noise tend to have higher CG-score. 
    (b) Fraction of label noise ($y$-axis) included in the examined portion ($x$-axis) for 20\% label noise. CG-score (blue) achieves better noise detectability for FMNIST than for CIFAR-100.}
    \label{fig:noise_detection}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/noise_exp/noise_detection_high.tex <==
\begin{figure*}[!tb]
\centering
    {\includegraphics[width=0.8 \linewidth]{fig/noise_exp/noise_detection_50.png}}\\
    {\includegraphics[width= 0.8\linewidth]{fig/noise_exp/noise_detection_80.png}}
    \caption{Fraction of label noise (y-axis) included in the examined portion (x-axis) for 50\%(top) and 80\%(bottom) label noise for FMINST  (left) and CIFAR-100 (right) datasets.}
    \label{fig:noise_detection_high}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/noise_exp/noisy_window.tex <==
%\begin{figure*}[!tb]
%\centering
%    {\includegraphics[width=0.3 \linewidth]{fig/noise_exp/noisyFMNIST_window.png}}
%    {\includegraphics[width=0.3 \linewidth]{fig/noise_exp/noisyCIFAR10_window.png}}
%    {\includegraphics[width=0.28 \linewidth]{fig/noise_exp/scatter_clean_noisy.png}}
%    \caption{
%    \change{(a) Window experiments with 20\% label noisy FMNIST(left) and CIFAR-10(middle) dataset.
%    The test accuracy of model trained with sub-datasets, which consist of data whose score order are between offset and offset+50\%. (b) Scatter graph of Partial CG-score (x axis) and CG-score (y axis) of 20\% noisy CIFAR10 dataset.}}
%    \label{fig:noisy_window}
%\end{figure*}

\begin{figure*}[!tb]
\centering
	\subfloat[Window experiment (FMNIST) \label{fig:window_a}]{\includegraphics[width=0.33\linewidth]{fig/noise_exp/noisyFMNIST_window.png}}
    \subfloat[Window experiment (CIFAR-10)    \label{fig:window_b}]{\includegraphics[width=0.33\linewidth]{fig/noise_exp/noisyCIFAR10_window.png}}
    \subfloat[Scatter graph (CIFAR-10) \label{scatter_c}]{\includegraphics[width=0.32\linewidth]{fig/noise_exp/scatter_clean_noisy.png}}
    \caption{(a) and (b) Window experiments with 20\% label noisy for FMNIST (a) and CIFAR-10 (b) datasets.
    Test accuracy (y-axis) of a model trained with 50\% of training instances selected from offset\% (x-axis) to (offset+50)\% scoring group. %The test accuracy of model trained with sub-datasets, which consist of data whose score order are between offset and offset+50\%. 
    (c) Scatter graph of Partial CG-score (x-axis) and CG-score (y-axis) for CIFAR-10 with 20\% label noise.
    }
    \label{fig:noisy_window}
\end{figure*}



==> ICLR2023_CGscore (CameraReady)/fig/noise_exp/score_distribution.tex <==
\begin{figure*}[!tb]
\centering
    {\includegraphics[width=0.96 \linewidth]{fig/noise_exp/data_distribution_clean.png}}
    \\
    {\includegraphics[width=0.96\linewidth]{fig/noise_exp/data_distribution_labelnoise.png}}
    \caption{Density of CG-scores at clean dataset and label noisy dataset.}
    \label{fig:score_distribution}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/pruning_exp/pruning_exp.tex <==
\begin{figure*}[!tb]
\centering
    \begin{tabular}{c}
	    \subfloat[Pruning low-scoring examples first. Better score maintains the test accuracy longer. ]
	    {{\includegraphics[height=2.5cm, width=0.275\linewidth]{fig/pruning_exp/pruning_FMNIST_resnet18.png}}
	    {\includegraphics[height=2.5cm, width=0.25\linewidth]{fig/pruning_exp/pruning_CIFAR10_resnet18.png}}
	    {\includegraphics[height=2.5cm, width=0.25\linewidth]{fig/pruning_exp/pruning_CIFAR100_resnet50.png}}}
	    \\ 
	    \subfloat[Pruning high-scoring examples first. Better score makes the rapid performance drop.]
	    {{\includegraphics[height=2.35cm, width=0.275\linewidth]{fig/pruning_exp/pruning_FMNIST_resnet18_rev.png}}
	    {\includegraphics[height=2.35cm, width=0.25\linewidth]{fig/pruning_exp/pruning_CIFAR10_resnet18_rev.png}}
	    {\includegraphics[height=2.35cm, width=0.25\linewidth]{fig/pruning_exp/pruning_CIFAR100_resnet50_rev.png}}}
    \end{tabular}
    \caption{
    Pruning experiments with FMNIST (left), CIFAR-10 (middle) and CIFAR-100 (right). 
    Only CG-Score does not require any training of the model to calculate the scores, but it achieves competitive performances and outperforms the random baseline. In (a), CG-score maintains the test accuracy up to significant removing portions; in (b), the test accuracy drops most rapidly for CG-score since the examples with high CG-score are essential in generalization of the model. 
 %   Final test accuracy according to the amount of training data for each score. The first row is the final test accuracy when pruning data with low values, and the second is the final test accuracy when pruning data with high values(labeled to the left). Each column is arranged according to which training data is used(labeled above).
    }
    \label{fig:pruning_exp}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/smallCIFART10.tex <==
\begin{figure*}[!tb]
\centering
	{\includegraphics[width=0.49\linewidth]{fig/small_cifar10_Spearmanr.png}}
	{\includegraphics[width=0.49\linewidth]{fig/small_cifar10_Pearson.png}}
	\caption{We create Small CIFAR-10 dataset by sampling 1,000 data from each class of CIFAR-10 dataset. Figures show Spearman's rank correlation(left) and Pearson correlation(right) between the CG-score of Small CIFAR-10 and CG-score calculated by subsampling the dataset (stochastic CG-score) as the number of calculations (random sampling) increases.
	Stochastic CG-scores are calculated with 2,000 (cyan), 3,000 (orange), 4,000 (green), and 5,000 (red) instances, while the full data includes 10,000 instances (1,000 for each class).
    X-axis indicates the number of independent runs to calculate averaged score, and Y-axis indicates the correlations.
    }
    \label{fig:smallCIFAR10}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/visualize_exp/CIFAR_mean_std.tex <==
\begin{figure*}[!tb]
\centering
	{\includegraphics[width=0.47\linewidth]{fig/visualize_exp/CIFAR100_means_std.png}}
	\label{fig:CIFAR100_means_std}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/visualize_exp/Imagenet.tex <==
\begin{figure*}[!htb] 
\centering
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/Imagenet_figure.png}}
    \\
    \subfloat[Examples and histograms of four classes in Imagenet\label{fig:imagenet_means_four}]
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/Imagenet_hist.png}}
    % \hfill
    % \subfloat[CIFAR100-Flatfish \label{fig:Frog}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_bottle_hist.png}}
    % \hfill
    % \subfloat[CIFAR10-Orange \label{fig:Truck}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_orange_hist.png}}
    % \subfloat[CIFAR10-plain \label{fig:Truck}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_plain_hist.png}}
    
    \caption{\change{Sample analysis for Imagenet in terms of the CG-score. Figure shows 4 top-ranked examples (top rows) and 4 bottom ranked examples (bottom rows) for Cypripedium, Oxcart, Orange, and Horn classes of Imagenet dataset. Histograms show distributions of the CG-scores for each class.}}
\label{fig:visualize_Imagenet}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/visualize_exp/visualize_exp.tex <==
% \begin{figure*}[!tb]
% \centering
% 	\subfloat[Top-ranked in CG score examples in CIFAR10 \label{fig:visualize_high}]{\includegraphics[width=0.49\linewidth]{fig/visualize_exp/high_vi.png}}
%     \subfloat[Bottom-ranked in CG score examples in CIFAR10 \label{fig:visualize_low}]{\includegraphics[width=0.49\linewidth]{fig/visualize_exp/low_vi.png}}
%     \caption{(a) Three top-ranked CG score examples by class. We observe that some top-ranked examples have large, positive $y_i( \rvy_{-i}^\top\rvh_i)$ value. This indicates that some top-ranked samples are classified as data with the noisy label in equation \ref{eqn:ab_trend}. We annotate these noisy label data in the red box. 
%     (b) Three bottom-ranked CG score examples by class.}
%     \label{fig:visualize_exp}
% \end{figure*}

\begin{figure*}[!tb]
\centering
	\subfloat[Examples of MNIST dataset \label{fig:visualize_MNIST}]{\includegraphics[width=0.49\linewidth]{fig/visualize_exp/MNIST_picture_.png}}
    \subfloat[Examples of FMNIST dataset \label{fig:visualize_FMNIST}]{\includegraphics[width=0.49\linewidth]{fig/visualize_exp/FMNIST_picture_.png}}
    \\
    \subfloat[Examples of CIFAR-10 dataset (Cat, dog, frog, and truck) \label{fig:visualize_CIFAR10}]{\includegraphics[width=0.98\linewidth]{fig/visualize_exp/CIFAR10_image_.png}}\\
    \caption{Examples sorted by CG-score. In (a) and (b), top-3 rows / bottom-3 rows display top-ranked / bottom-ranked examples, respectively. Among top-ranked examples, (possibly) mislabeled examples are marked by red rectangles. In (c),  top-2 rows / bottom-2 rows display top-ranked / bottom-ranked examples, respectively.}
    \label{fig:visualize_exp}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/visualize_exp/visualize_exp_CIFAR10.tex <==
\begin{figure*}[!tb] \label{fig:CIFAR10_image_hist_}
\centering

	{\includegraphics[width=1\linewidth]{fig/visualize_exp/CIFAR10_image_.png}}
    \\
    %{\includegraphics[width=1\linewidth]{fig/visualize_exp/CIFAR10_image_hist_.png}}
    \caption{Top-ranked examples (top two rows) and bottom ranked examples(bottom two rows) for four classes of CIFAR-10 dataset.}
    \label{fig:visualize_exp_CIFAR10}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/visualize_exp/visualize_exp_CIFAR100.tex <==
\begin{figure*}[!tb] \label{fig:CIFAR100_image_hist_}
\centering
    \subfloat[Distribution of CG-scores at CIFAR-100\label{fig:CIFAR100_means_std}]
	{\includegraphics[width=0.5\linewidth]{fig/visualize_exp/CIFAR100_means_std.png}}
	\\
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/CIFAR100_image_.png}}
    \\
    \subfloat[Examples and histograms of four classes in CIFAR-100 \label{fig:visualize_exp_CIFAR100}]
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/CIFAR100_image_hist_.png}}
    % \hfill
    % \subfloat[CIFAR100-Flatfish \label{fig:Frog}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_bottle_hist.png}}
    % \hfill
    % \subfloat[CIFAR10-Orange \label{fig:Truck}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_orange_hist.png}}
    % \subfloat[CIFAR10-plain \label{fig:Truck}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_plain_hist.png}}
    
    \caption{Sample analysis for CIFAR-100 dataset in terms of the CG-score. (a) shows the CG-score means and standard deviations of 100 classes in CIFAR-100 dataset. (b) shows ten top-ranked examples (top two rows) and ten bottom ranked examples (bottom two rows) for orange, plain, bottle, and flatfish classes of CIFAR-100 dataset. Histograms show distributions of the CG-scores for each class.}
    \label{fig:app:cifar100}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/fig/visualize_exp/visualize_exp_imagenet.tex <==
\begin{figure*}[!htb] 
\centering
    \subfloat[Distribution of CG-scores at ImageNet\label{fig:Imagenet_means_std}]
	{\includegraphics[width=0.5\linewidth]{fig/visualize_exp/Imagenet_mean_std.png}}
	\\
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/Imagenet_figure.png}}
    \\
    \subfloat[Examples and histograms of four classes in Imagenet\label{fig:Imagenet_means_four}]
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/ImageNet_hist.png}}

    
    \caption{Sample analysis for ImageNet in terms of the CG-score. (a) shows the CG-score means and standard deviations of 1,000 classes in ImageNet dataset. (b) shows four top-ranked examples (top row) and four bottom ranked examples (bottom row) for Jack-o-lantern, Rapeseed, Ladybug, and Spatula classes of ImageNet dataset. Histograms show density distributions of the CG-scores for each class.}
\label{fig:visualize_Imagenet}
\end{figure*}

==> ICLR2023_CGscore (CameraReady)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR2023_CGscore (CameraReady)/section/0_abstract.tex <==
\begin{abstract}
Many recent works on understanding deep learning try to quantify how much individual data instances influence the optimization and generalization of a model. %, either by analyzing the behavior of the model during training or by measuring the performance gap of the model when the instance is removed from the dataset. 
Such attempts reveal characteristics and importance of individual instances, which may provide useful information in diagnosing and improving deep learning. However, most of the existing works on data valuation require actual training of a model, which often demands high-computational cost.
%sometimes contradicts the motivation for data valuation --- for example, when one wants to select and use only a subset of data instances that are important in training to save the computational cost, one first needs to train the model with the full dataset to identify the samples to prune without a large sacrifice in performance. 
In this paper, we provide a training-free data valuation score, called {\it complexity-gap score}, which is a data-centric score to quantify the influence of individual instances in generalization of two-layer overparameterized neural networks. The proposed score can quantify irregularity of the instances and measure how much each data instance contributes in the total movement of the network parameters during training. %We theoretically analyze and empirically demonstrate the correlation of the proposed score with other scores defined using the information from training dynamics. 
We theoretically analyze and empirically demonstrate the effectiveness of the complexity-gap score in finding `irregular or mislabeled' data instances, and also provide applications of the score in analyzing datasets and diagnosing training dynamics. Our code is publicly available at \url{https://github.com/JJchy/CG_score}.
\end{abstract}

==> ICLR2023_CGscore (CameraReady)/section/1_intro.tex <==
\section{Introduction}\label{sec:intro}

Creation of large datasets has driven development of deep learning in diverse applications including computer vision \citep{cnn, ViT}, natural language processing \citep{transformer, gpt3} and reinforcement learning \citep{dqn, alphago}. 
To utilize the dataset in a more efficient and effective manner, some recent works have attempted to understand the role of {\it individual} data instances in training and generalization of neural networks. 
In~\citep{shapley}, a metric to quantify the contribution of each training instance in achieving a high test accuracy was analyzed under the assumption that not only the training data but also the test data is available. 
\citet{cscore} defined a score to identify irregular examples that need to be memorized during training, in order for the model to accurately classify the example.  
%\citet{carto}, on the other hand, analyzed the characteristics of data instances with respect to their role in out-of-distribution generalizations. 
%A promising attempt to decompose the role of individual data instance in training a model is {\it data valuation}, where the goal is to quantify the impact of data in algorithmic predictions and decisions. 

All these previous methods for data valuation require {\it actual training} of a model to quantify the role of individual instances at the model. 
Thus, the valuation itself often requires high-computational cost, which may contradict some motivations of data valuation.
For example, in~\citep{shapley,cscore}, to examine the effect of individual data instances in training, one needs to train a model repeatedly while eliminating each instance or subsets of instances. %, which requires training of a model at least the number of times proportional to the number of training instances. 
In \citep{carto, forgetting}, on the other hand, training dynamics--the behavior of a model on each instance throughout the training--is analyzed to categorize data instances. %, which also requires the training of a model with the full dataset. 
When the motivation for data valuation lies at finding a subset of data that can approximate the full-dataset training to save the computational cost for training, the previous valuation methods might not be suitable, since they already require the training with the full dataset before one can figure out `important' instances. % and possibly prune the rest of the examples. % that do not significantly degrade the generalization of the model. 
%data valuation is useful: pruning, irregularities, effect of memorization, analysis of training dynamics
%current methods: categories, all computational cost, for pruning application, already require some training using the full datasets
%our method: we propose training-free data valuation. Still it has a close connection to the generalization of neural network, since the measure is defined by the algorithm-dependent generalization measure. Implications in training dynamics. Geometric interpretation, demonstrate the effectiveness of the score as data value. Application of the score. 




In this paper, our main contribution is on defining a {\it training-free} data valuation score, which can be directly computed from data and can effectively quantify the impact of individual instances in optimization and generalization of neural networks. The proposed score, called {\it complexity-gap score}, measures the gap in {\it data complexity} where a certain data instance is removed from the full dataset.
The data complexity measure was originally introduced in \cite{arora2019fine} to quantify the complexity of the full dataset, which was used in bounding the generalization error of overparameterized two-layer neural networks trained by gradient descent. Different from that work, where the complexity of the full dataset was of main concern, our focus is on decomposing the effect of individual data instances in the training, and thus we newly introduce a complexity gap score (CG-score). 
We theoretically analyze and empirically demonstrate that the CG-score can quantify `irregularity' of instances within each class, and thus can be used in identifying atypical examples, either due to the inherent irregularity of the instance or mislabeled classification. We also demonstrate that the proposed score has a close relation to `learning difficulty' of the instances by analyzing the training dynamics of data instances. 
Our key contributions are as below:
\begin{itemize}%[leftmargin=-.5in]
\item {\it Training-free data valuation:} Different from previous methods for data valuation, most of which leverage the information from training itself, we provide a training-free data valuation score, CG-score, which is the data-centric score to quantify the effect of individual data instances in optimization and generalization of neural networks. %The complexity-gap score measures how much each data instance contributes in the total movement of the network parameters, which is also related to the gap in generalization bounds when the data instance is removed from the dataset.
\item {\it Geometric interpretation:} We provide analysis that the CG-score can measure {\it irregularity} of each instance, i.e., it measures the average `similarity' of an instance to the instances of the same class and the average `dissimilarity' to the instances of different classes. %how much each instance represents the instances of the same class and how much it is different from those of other classes. %We also show that samples with label noise tend to have higher complexity-gap score. %By both synthetic and real dataset experiments, we demonstrate these findings. 
\item {\it Effectiveness of the score}: We empirically demonstrate the effectiveness of the CG-score in data valuation. We show that pruning data instances with small CG-score does not significantly degrade the generalization capability of a model, e.g., for CIFAR-10 we can prune 40\% of the data with less than 1\% of drop in test accuracy. Our scoring method is especially useful in data pruning, since different from other scores, which require the training with the full dataset, our method does not require any training of a model. 
\item {\it Application of the score:} We provide potential applications of the CG-score in analyzing datasets and training dynamics. We analyze the histograms of the CG-score for various datasets to demonstrate that the CG-score can measure irregularity of the instances. We also demonstrate that the instances with higher CG-score are `difficult' examples, which are learned slowly by the models, by comparing the loss and test accuracy curves and the evolution of Neural Tangent Kernel (NTK) submatrices of lowest/highest-scoring groups.
\end{itemize}

==> ICLR2023_CGscore (CameraReady)/section/2_related.tex <==
\section{Related Works}\label{sec:related}

%\paragraph{Deep learning analysis from instance perspective}

Different from many existing works where the effect of datasets on model training is analyzed as a whole, some recent works have focused on understanding the impact of individual data instances. 
\cite{shapley,Dshapley} defined `Data Shapley', to evaluate the value of each data instance, by measuring the average gap in performances when an instance is held-out from any subsets of a given training data.
\cite{cscore} defined consistency score (C-score) of each instance by estimating the prediction accuracy of the instance attained by the model trained with the full dataset except the instance. Both Data Shapley and C-score require multiple trainings of a model to compute the scores. Another main branch uses the training dynamics to identify `difficult' instances for classification, either due to irregularity or mislabeling, by measuring different forms of {\it confidence, stability or influence} in the decision of the networks throughout the training \citep{forgetting, carto, tracin}. In \citep{depth}, the computational difficulty of an instance is defined as the number of hidden layers after which the networks' prediction coincides with the prediction at the output. With application of robust learning, some works quantify the difficulty of each instance by a `margin' from the decision boundary %, which can be measured by the amount of noise sufficient to alter the decision of the network when the noise is added to the instance  
 \citep{margin}. 
CRAIG \citep{CRAIG} finds valuable subsets of data as coresets that preserve the gradient of the total loss.
All these previous methods are demonstrated to be effective in at least one or more applications of data valuation, including data pruning \citep{EL2N, carto, VoG, mem}, importance-based weighted sampling \citep{activebias, infl_func}, noise filtering \citep{dividemix, RoG, FINE}, robust learning \citep{learnreweight, AUM}, out-of-distribution generalizations \citep{carto} or diverse sample generalization \citep{lee2021self}. However, all these methods require the training of a model with the full dataset (at least for a few optimization steps). % or possibly for as many times as the number of instances in the training dataset. 
Recently, some works try to evaluate different subsets of training data by utilizing generalization error bound, induced by the NTK theory of neural networks \citep{DaVinZ, rethink}. However, these methods do not provide a computationally-efficient way to quantify the effect of individual data instances.
Our data valuation method, on the other hand, is a data-centric method that can be efficiently calculated from data only without training of a model. %We demonstrate that with our scoring method, we can effectively analyze the impact of individual data instance in optimization and generalization of neural networks.


%learning view: 
%\cite{curricula} learning speed
%\cite{carto} OOD generalization
%\cite{forgetting} forgetting
%Also, has close relation to robust learning against noise labels \cite{ELR}

%computational view:
%\cite{depth} prediction depth

%geometric view:
%\cite{margin} margin (how difficult it is to attack the natural data point, geometry-aware learning) robust learning


%main them - finding difficult samples, treat them differently, help deep learning training and generalization
%pruning less important data, 
%emphasizing more important data by score-based reweighting

%But all the methods require model training
%purely geometry-based measure often fails since the valuation needs to consider the algorithm
%our measure data complexity gap score, defined using the algorithm dependent data complexity measure from \cite{arora2019fine}

%Optimization and traing dynamics of 2-layer overparameterized network can be explained with gram matrix. (papers)
%\paragraph{Data valuation from training dynamics}



==> ICLR2023_CGscore (CameraReady)/section/3_score.tex <==
\section{Complexity-Gap Score: Data Valuation without Training}\label{sec:score}
In this section, we introduce a new data valuation score, called {\it complexity-gap score}, based on the analysis of overparameterized two-layer neural networks from \citet{arora2019fine}.%which captures the effect of each data instance in optimization and generalization for overparameterized two-layer neural networks.  %The score we introduce 
%can be directly and efficiently calculated from given data, without the need of training neural networks. 

\subsection{Preliminaries: data complexity measure in two-layer neural networks}

We first review the result from \citet{arora2019fine}, where a two-layer neural network trained by randomly initialized gradient descent is analyzed. 
%In the paper, the generalization bound is derived based on a data-dependent complexity measure. 
%The data complexity measure is the complexity of the whole dataset that governs the amount of total movement of all neurons during training of neural networks. In this paper, we will introduce a {\it complexity-gap score}, which is the gap between the data complexity measure with and without a certain data instance, to decompose the effect of individual data instance in optimization and generalization of neural networks.
%Following the notations from \citet{arora2019fine}, we c
Consider a two-layer ReLU activated neural network having $m$ neurons in the hidden layer, of which the output is $f_{\rmW,\rva}(\rvx)=\frac{1}{\sqrt{m}}\sum_{r=1}^m a_r \sigma(\rvw_r^\top \rvx)$ where $\rvx\in\R^{d}$ is the input, $\rvw_1,\dots, \rvw_m\in\R^{d}$ are weight vectors in the first layer, $a_1,\dots, a_m\in \R$ are weights in the second layer, and $\sigma(x)=\max(0,x)$ is the ReLU activation function. Let $\rmW=(\rvw_1,\dots, \rvw_m)\in \R^{d\times m}$ and $\rva=(a_1,\dots, a_m)^{\top}\in\R^{m}$. Assume that the network parameters are randomly initialized as $\rvw_r(0)\sim \mathcal{N}(0,\kappa^2I_{d\times d})$ and $a_r \sim \text{unif}(\{-1,1\})$, $\forall r\in[m]$, where $\kappa \in(0,1]$ is the size of random initialization. The second layer $\rva$ is then fixed and only the first layer $\rmW$ is optimized through gradient descent (GD) to minimize the quadratic loss, $\Phi(\rmW)=\frac{1}{2}\sum_{i=1}^n (y_i-u_i)^2$ where $u_i=f_{\rmW, \rva}(\rvx_i)$ and $\{(\rvx_i,y_i)\}_{i=1}^n$ is the dataset drawn i.i.d. from an underlying distribution $\mathcal{D}$. 
The GD update rule can be written as $\rvw_r(k+1)-\rvw_r(k)=-\eta \frac{\partial \Phi(\rmW(k))}{\partial \rvw_r}$ where $\eta>0$ is the learning rate.
The output of the network for the input $\rvx_i$ at the $k$-th iteration is denoted by $u_i(k)=f_{\rmW(k),\rva}(\rvx_i)$.
For simplicity, it is assumed that $\|\rvx\|_2=1$ and $|y|\leq 1$. 

The data complexity measure governing the training of the two-layer ReLU activated neural network is defined in terms of the following {\it Gram matrix} $\rmH^\infty\in \R^{n\times n}$ associated with ReLU activation:
\beq
\begin{split}\label{eqn:gram}
\rmH_{ij}^\infty&=\E_{\bsw\sim \mathcal{N}(0,I_{d\times d})}\left[\rvx_i^\top \rvx_j \mathbbm{1}\{\rvw^\top \rvx_i\geq0, \rvw^\top \rvx_j\geq 0\} \right]=\frac{\rvx_i^\top \rvx_j(\pi-\arccos(\rvx_i^\top \rvx_j))}{2\pi}.
\end{split}
\eeq
In \citet{arora2019fine}, a complexity measure of data was defined as $\rvy^\top (\rmH^\infty)^{-1} \rvy$ where $\rvy=(y_1,\dots,y_n)$, and it was shown that this measure bounds the total movement of all neurons in $\rmW$ from their random initialization. Moreover, the data complexity measure bounds the generalization error by restricting the Rademacher complexity of the resulting function class. In the following, we write the eigen-decomposition of $\rmH^\infty$ as $\rmH^\infty=\sum_{i=1}^n \lambda_i \rvv_i \rvv_i^\top$ where $\lambda_i$'s are ordered such that $\lambda_1\geq \lambda_2\geq \dots \lambda_n$. Further, assuming  $\lambda_n\geq\lambda_0>0$, we can write $(\rmH^\infty)^{-1}=\sum_{i=1}^n (\lambda_i)^{-1} \rvv_i \rvv_i^\top$.
\begin{thm}[Informal version of \citep{arora2019fine}]\label{thm:arora} Assume that $\lambda_{\min}(\rmH^\infty)=\lambda_n\geq\lambda_0>0$. For sufficiently large width $m$, sufficiently small learning rate $\eta>0$ and sufficiently small random initialization $\kappa>0$, with probability at least $1-\delta$ over the random initialization, we have 
\beq
\begin{split}\nonumber
%&\text{a) Bound in loss}: \vy-\vu(k)=(I-\eta \mH^{\infty})^k \vy+\text{small constant}\\
&\text{a) Bound in loss}: \|\rvy-\rvu(k)\|_2=\sqrt{\sum_{i=1}^n (1-\eta \lambda_i)^{2k}(\rvv_i^\top \rvy)^2}+\text{small constant},\\
&\text{b) Bound in total movement of neurons: } \|\rmW(k)-\rmW(0)\|_F\leq \sqrt{\rvy^\top(\rmH^\infty)^{-1} \rvy}+\text{small constant},\\
&\text{c) Bound in population loss: }\E_{(\rvx,y)\sim \mathcal{D}}[l(f_{\rmW(k),\rva}(\rvx),y)]\leq \sqrt{\frac{\rvy^\top(\rmH^\infty)^{-1} \rvy}{n}}+O\left(\sqrt{\frac{\log\frac{n}{\lambda_0\delta}}{n}}\right),
\end{split}
\eeq
where a) and b) hold for all iteration $k\geq 0$ of GD, and c) holds for $k\geq \Omega\left({1}/{(\eta \lambda_0)}\log({n}/{\delta})\right)$.
\end{thm}
This theorem shows that if the label vector $\rvy$ is aligned with top eigenvectors of $\rmH^\infty$,  i.e., $(\rvv_i^\top \rvy)$ is large for large $\lambda_i$, then the loss decreases quickly and the total movement of neurons as well as the generalization error is small. 
Thus, the data complexity measure $\rvy^\top(\rmH^\infty)^{-1} \rvy$ captures the complexity of data governing both the optimization and generalization of the overparameterized two-layer neural networks. However, this quantity captures the complexity of the whole data. To decompose the effect of individual instances, we newly define a {\it complexity-gap score}.
 
\subsection{Complexity-gap score and training dynamics}

We define the {\it complexity-gap score} (CG-score) of $(\rvx_i, y_i)$ as the difference between the data complexity measure when $(\rvx_i, y_i)$ is removed from a given dataset  $\{(\rvx_i,y_i)\}_{i=1}^n$:
\beq\label{def:vi}
\mathrm{CG}(i)=\rvy^\top (\rmH^\infty)^{-1} \rvy-\rvy_{-i}^\top (\rmH_{-i}^\infty)^{-1} \rvy_{-i}
\eeq
 where $\rvy_{-i}$ is the label vector except the $i$-th sample point and $\rmH_{-i}^{\infty}$ is the $(n-1)\times (n-1)$ matrix obtained by removing the $i$-th row and column of $\rmH^\infty$.
 
We first emphasize that the proposed score can be easily calculated from given data without the need of training neural networks, as opposed to other data valuation scores requiring either a trained neural network or statistics calculated from training dynamics. Yet, the proposed score captures two important properties on the training and generalization of data instance, implied by Theorem \ref{thm:arora}:
\begin{enumerate}
\item An instance $(\rvx_i,y_i)$ with a large CG-score is a `difficult' example, in the sense that removing it from the dataset reduces the generalization error bound by a large amount, which implies that the dataset without $(\rvx_i,y_i)$ is much easier to be learned and generalized. 
\item  An instance $(\rvx_i,y_i)$ with a larger CG-score contributes more on the optimization and drives the total movement of neurons by a larger amount, measured by $ \|\rmW(k)-\rmW(0)\|_F$. 
\end{enumerate}

We next discuss the computational complexity of calculating the CG-score.
To calculate $\{\mathrm{CG}(i)\}_{i=1}^n$, we need to take the inverse of matrices $\rmH^\infty$ and $\rmH_{-i}^\infty$ for all $i\in[n]$, which requires $O(n^4)$ complexity when we use general $O(n^3)$-complexity algorithm for the matrix inversion.
By using Schur complement, however, we can reduce this complexity to $O(n^3)$. %, since $(\rmH_{-i}^\infty)^{-1}$ can be easily calculated from $(\rmH^\infty)^{-1}$ for all $i\in[n]$. 
Without loss of generality, we can assume $i=n$. 
Denote $\rmH^\infty$ and $(\rmH^\infty)^{-1}$ by
\beq\label{eqn:mtr_notation}
\rmH^\infty=\begin{pmatrix}  \rmH_{n-1}^\infty & \rvg_{i} \\ \rvg_i^\top &c_i\end{pmatrix}, \quad
(\rmH^\infty)^{-1}=\begin{pmatrix}  (\rmH^\infty)^{-1}_{n-1}  & \rvh_{i} \\ \rvh_i^\top&d_i \end{pmatrix},
\eeq
where $\rmH^\infty_{n-1}, (\rmH^\infty)^{-1}_{n-1} \in \mathbb{R}^{(n-1)\times (n-1)}$, $\rvg_i, \rvh_i\in \mathbb{R}^{n-1}$ and $c_i,d_i\in\mathbb{R}$.
%where $\rmH^\infty_{n-1}$ and $(\rmH^\infty)^{-1}_{n-1}$ denote the $(n-1)\times (n-1)$ upper submatrix of $\rmH^\infty$  and $(\rmH^\infty)^{-1}$, respectively,  $\rvg_i=\rmH^\infty_{1:(n-1),n}$ and $\rvh_i=(\rmH^\infty)^{-1}_{1:(n-1),n}$ denote the first $(n-1)$-entires of the $n$-th column of $\rmH^\infty$ and $(\rmH^\infty)^{-1}$, respectively, and $c_i=H^\infty_{n,n}$ and $d_i=(H^\infty)^{-1}_{n,n}$ denote the $(n,n)$-th entry of  $\rmH^\infty$ and $(\rmH^\infty)^{-1}$, respectively.
From $\rmH^\infty (\rmH^\infty)^{-1}=\mI_{n}$, we have $\rvg_i^\top (\rmH^\infty)^{-1}_{n-1}+c_i \rvh_i^\top=0$, i.e., $\rvh_i^\top=-c_i^{-1} \rvg_i^\top (\rmH^\infty)^{-1}_{n-1}$.

By Schur complement, $(\rmH_{-i}^\infty)^{-1}$, which is equal to $(\rmH^\infty_{n-1})^{-1}$ for $i=n$, can be calculated as
\beq\label{eqn:Shur}
(\rmH_{-i}^\infty)^{-1}= (\rmH^\infty)^{-1}_{n-1}-d_i^{-1}\rvh_i \rvh_i^\top.
\eeq
Since we have 
\beq
\begin{split}
\rvy^\top (\rmH^\infty)^{-1} \rvy&=\rvy_{-i}^\top (\rmH^\infty)^{-1}_{n-1} \rvy_{-i} + y_i \rvh_i^\top \rvy_{-i}+y_i \rvy_{-i}^\top \rvh_i+y_i^2 d_i,\\
\rvy_{-i}^\top (\rmH_{-i}^\infty)^{-1} \rvy_{-i}&=\rvy_{-i}^\top (\rmH^\infty)^{-1}_{n-1} \rvy_{-i}-d_i^{-1}(\rvy_{-i}^\top \rvh_i)^2,
\end{split}
\eeq
the CG-score, $\mathrm{CG}(i)$ in \eqref{def:vi}, can be calculated by
\beq\label{eqn:vi_simp}
\mathrm{CG}(i)= d_i^{-1}(\rvy_{-i}^\top\rvh_i)^2+2y_i( \rvy_{-i}^\top\rvh_i )+y_i^2 d_i=\left({(\rvy_{-i}^\top\rvh_i)}/{\sqrt{d_i}}+y_i\sqrt{d_i}\right)^2.
\eeq
Thus, $\mathrm{CG}(i)$ can be calculated by the $n$-th column $(\rvh_i, d_i)$ of $(\rmH^\infty)^{-1}$, without the need of calculating $(\rmH^\infty_{-i})^{-1}$ when $i=n$.
The case for general $i\neq n$ can also be readily solved by permuting the $i$-th row and column of $\rmH^\infty$ into the last positions. 
 
 
\paragraph{Correlation to other scores}
We show relation between our score and other data valuation scores that require the training of neural networks. 
\citet{forgetting} define `the forgetting score' for each training example as the number of times during training the decision of that sample switches from a correct one to incorrect one. 
\citet{EL2N}, on the other hand, suggest the GraNd score, which is the expected loss gradient norm $\E[\|\nabla_{\rmW(k)} l(u(k),y) \|]$, to bound the contribution of each training example to the decrease of loss on any other example over a single gradient step. 
 The GraNd score is further approximated (under some assumptions) by the EL2N score, defined to be $\E[|y-u(k)|]$ where $u(k)$ is the output of the neural network for the sample $(x,y)$ at the $k$-th step.
 Since $|y-u(k)|$, if rescaled, is an upper bound on 0--1 loss, $\sum_k|y-u(k)|$ upper bounds forgetting score after rescaling. Thus, an example with a high forgetting score will also have a high GraND score and high EL2N score averaged over multiple time steps.
We next relate our complexity-gap score to $\sum_k (y-u(k))$, and thus to all the three previous scores defined using training dynamics.

It was shown in \citep{arora2019fine} that for the overparameterized two-layer networks trained by GD, the gap between the label vector and the network output at the step $k$ can be approximated as $\rvy-\rvu(k)\approx (I-\eta \rmH^\infty)^k \rvy$. Thus, we get $\sum_{k=0}^\infty \rvy-\rvu(k)\approx \sum_{k=0}^\infty  (I-\eta \rmH^\infty)^k \rvy=\frac{1}{\eta} (\rmH^\infty)^{-1}\rvy$. Without loss of generality, consider $i=n$. Then, the accumulated difference between $y_i$ and $u_i(k)$ over $k$ can be approximated as 
\beq\label{eqn:acc}
\sum_{k=0}^\infty (y_i-u_i(k))\approx \left( \rvh_i^\top \rvy_{-i}+y_i d_i\right)/\eta=\left(  \rvy_{-i}^\top  \rvh_i/\sqrt{d_i}+y_i \sqrt{d_i} \right)\sqrt{d_i}/\eta.
\eeq
Note that both the right-hand side of \eqref{eqn:acc} and $\mathrm{CG}(i)$ in \eqref{eqn:vi_simp} depend on the term $\left(  \rvy_{-i}^\top  \rvh_i/\sqrt{d_i}+y_i \sqrt{d_i} \right)$. Thus, we can expect that $\mathrm{CG}(i)$ will be correlated with the scores related to training dynamics, including the forgetting score, GraND score and EL2N score. Different from those scores, our score can be directly calculated from the data without training of a model. %When we want to use the data valuation score to select important examples and to prune the rest of the examples in order to save the memory and computational resource in training of neural networks, the CG-score CG(i) can be especially useful since it does not require any actual training using the high-volume of the dataset.

\input{table/rank_corr}

\paragraph{Inversion of $\rmH^\infty$ is an effective step}
In the definition of $\mathrm{CG}(i)$ in \eqref{def:vi}, we use the inverse of $\rmH^\infty$ to measure the alignment of the eigenvectors of $\rmH^\infty$ with the label vector $\rvy$. One could suggest another score that directly uses $\rmH^\infty$ instead of $(\rmH^\infty)^{-1}$, which can save the computation for inversion.
However, we argue that the score calculated by using $(\rmH^\infty)^{-1}$ includes more information than the score calculated by $\rmH^\infty$ due to the reason described below. Let us define $\mathrm{CG'}(i):=\rvy^\top \rmH^\infty \rvy-\rvy_{-i}^\top \rmH_{-i}^\infty \rvy_{-i}$. Without loss of generality, assume $i=n$.  Then, $\mathrm{CG'}(i)=2y_i(\rvg_i^\top\rvy_{-i} )+y_i^2 c_i$ where $\rvg_i=(\rmH^\infty)_{1:(n-1),n}$ and $c_i=H^\infty_{n,n}$ as defined in \eqref{eqn:mtr_notation}. Since $c_i=1/2$ for all $i\in[n]$ from the definition of $\rmH^\infty$ in \eqref{eqn:gram} and $y_i^2=1$ for $y_i=\pm1$, we have $\mathrm{CG'}(i)=2(y_i (\rmH^\infty \rvy)_i-1/2)+1/2 $.
By using the approximation $\rvy-\rvu(k)\approx (I-\eta \rmH^\infty)^k \rvy$ from \citet{arora2019fine}, we have $\rvy-\rvu(1)\approx \rvy-\eta \rmH^\infty \rvy$ when $k=1$, which implies $\rvu(1)\approx \eta \rmH^\infty \rvy$. Thus, $\mathrm{CG'}(i)=\frac{2}{\eta} y_i u_i(1) +1/2$. Note that an instance $(\rvx_i,y_i)$ has a large $\mathrm{CG'}(i)$ if $y_iu_i(1)$ is large, i.e., the network output $u_i(1)$ after 1-time step has the same sign as the targeted label $y_i\in\{-1,1\}$ and has a large magnitude. Thus, $\mathrm{CG'}(i)$ measures how fast the training instance can be learned by the neural network. Different from $\mathrm{CG'}(i)$, our original score $\mathrm{CG}(i)$ is correlated with the accumulated error between $y_i$ and $u_i(k)$ averaged over the training as shown in \eqref{eqn:acc}. Thus, our original score $\mathrm{CG}(i)$, using the inverse of $\rmH^\infty$, reflects the statistics averaged over the whole training steps. 

In Table~\ref{tab:rank_corr}, we compare the Spearman'a rank correlation between CG-score/CG'-score and other data valuation scores including C-score \citep{cscore}, forgetting score \citep{forgetting} and EL2N score \citep{EL2N} for CIFAR-10/100 datasets.\footnote{The way we calculate CG-scores for multi-label datasets is explained in Appendix \S\ref{sec: multi-class}. To reduce the computation complexity, we calculated the scores by sub-sampling data and averaging them over multiple runs.} We can observe that CG-score has higher correlations with the previous scores compared to those of CG'-score. In the rest of this paper, we focus on the CG-score for our data valuation score. 



\subsection{Geometric interpretation of the complexity-gap score}\label{sec:geo_analysis}
\input{fig/gaussian_exp/gaussian_exp}
We next provide geometric interpretation for the CG-score. 
For the sake of simplicity, we consider binary dataset with $\frac{n}{2}$ samples having $y_i=1$ and $\frac{n}{2}$ samples having $y_i=-1$. We further assume that $\E[H_{ij}^\infty] =p$ if $y_i=y_j$ and $\E[H_{ij}^\infty]=q$ if $y_i\neq y_j$ for some $|p|>|q|$. %, i.e., if two samples $(\rvx_i, y_i)$ and $(\rvx_j, y_j)$ belong to the same class their inner product multiplied by $(\pi-\arccos(\rvx_i^\top \rvx_j))/2$ is high as $p$ compared to that of two samples from different classes, $q$. 
Note that the diagonal entires $H_{ii}^\infty=1/2$ for all $i\in[n]$.
Thus, $\E[\rmH^\infty]$ can be decomposed as $\E[\rmH^\infty]=\left(\frac{1}{2}-p\right)\mI_n+\mS$ where $\mS$ is a block matrix with $\mS=\begin{pmatrix}p& q\\ q& p\end{pmatrix}\otimes \mI_{n/2}$, and the resulting eigenvalues of $\E[\rmH^\infty]$ are $\frac{(p+q)n}{2}+\left(\frac{1}{2}-p\right)$, $\frac{(p-q)n}{2}+\left(\frac{1}{2}-p\right)$ and $\left(\frac{1}{2}-p\right)$ with multiplicity $(n-2)$. When $p=\Theta(q)$ and $p=o(1/n)$, the matrix $\E[\rmH^\infty]\approx (1/2)\mI_{n}$.
From the representations of $\rmH^\infty$ and $(\rmH^\infty)^{-1}$ in \eqref{eqn:mtr_notation} and the implied relation $\rvh_i^\top=-c_i^{-1} \rvg_i^\top (\rmH^\infty)^{-1}_{n-1}$, assuming $\rmH^\infty\approx (1/2)\mI_{n}$ and using $c_i=1/2$, we can write $\rvh_i^\top = - 4\rvg_i^\top$. By using this approximation, our CG-score in \eqref{eqn:vi_simp} can be approximated as
\beq\label{eqn:vi_simp_approx}
\mathrm{CG}(i)= d_i^{-1}(\rvy_{-i}^\top\rvh_i)^2+2y_i(  \rvy_{-i}^\top\rvh_i)+y_i^2 d_i\approx 8(y_i(\rvy_{-i}^\top\rvg_i))^2-8y_i(\rvy_{-i}^\top\rvg_i)+2
\eeq
since $d_i\approx 2$ and $y_i^2=1$. 
Since $y_i(\rvy_{-i}^\top\rvg_i)=\sum_{j\in\{[n]: y_i= y_j\}} H_{ij}^\infty-\sum_{j\in\{[n]: y_i\neq y_j\}} H_{ij}^\infty$ and
%\beq\label{eqn:ab_trend}
%\begin{split}
%y_i(\rvy_{-i}^\top\rvg_i)&=\sum_{j\in\{[n]: y_i= y_j\}} H_{ij}^\infty-\sum_{j\in\{[n]: y_i\neq y_j\}} H_{ij}^\infty\\
%&=\sum_{j\in\{[n]: y_i= y_j\}} \frac{\rvx_i^\top \rvx_j(\pi-\arccos(\rvx_i^\top \rvx_j))}{2\pi}-\sum_{j\in\{[n]: y_i\neq y_j\}}\frac{\rvx_i^\top \rvx_j(\pi-\arccos(\rvx_i^\top \rvx_j))}{2\pi},
%\end{split}
%\eeq
thus $\E[y_i(\rvy_{-i}^\top\rvg_i)]=\frac{(p-q)n}{2}=o(1)$, assuming $p=\Theta(q)$ and $p=o(1/n)$, the second term $-8y_i(\rvy_{-i}^\top\rvg_i)$ becomes much larger than the first term, which is proportional to $(y_i(\rvy_{-i}^\top\rvg_i))^2$. 
Thus, $-8y_i(\rvy_{-i}^\top\rvg_i)$ is the main term that determines the order of $\{\mathrm{CG}(i)\}_{i=1}^n$. 
Note that $y_i(\rvy_{-i}^\top\rvg_i)$ measures the gap between $\sum_{j\in\{[n]: y_i= y_j\}} H_{ij}^\infty$ and $\sum_{j\in\{[n]: y_i\neq y_j\}} H_{ij}^\infty$.
%the summation of $H_{ij}^\infty$ over the samples of the same class as $(\rvx_i,y_i)$ and that over the samples of the different class from $(\rvx_i,y_i)$. 
Since $H_{ij}^\infty=\frac{\rvx_i^\top \rvx_j(\pi-\arccos(\rvx_i^\top \rvx_j))}{2\pi}$,  $y_i(\rvy_{-i}^\top\rvg_i)$ measures the gap between the average similarities of $\rvx_i$ with other samples $\{\rvx_j\}$ of the same class $y_j=y_i$ and that with samples of the different class $y_j\neq y_i$, where the similarity is measured by the cosine between the two samples $(\rvx_i,\rvx_j)$ multiplied by the chance that ReLU is activated for both the samples.
Thus, we can expect two important trends regarding the CG-score:
\begin{enumerate}
\item Regular vs. irregular samples: If a sample $(\rvx_i,y_i)$ is a `regular' sample representing the class $y_i$ in the sense that it has a larger similarity with other samples of the same class than to samples from the different class, then it will have a large $y_i(\rvy_{-i}^\top\rvg_i)$, resulting in a lower CG-score due to the minus sign. On the other hand, if a sample  $(\rvx_i,y_i)$ is `irregular' in the sense that it does not represent the class and has a small similarity with the samples of the same class, then $y_i(\rvy_{-i}^\top\rvg_i)$ will be small, resulting in a higher CG-score.
%large $\rvx_i^\top \rvx_j$ with the samples of the same class $\{\rvx_j:y_j=y_i\}$ and has a small or negative $\rvx_i^\top \rvx_j$ with the samples of the different class $\{\rvx_j:y_j\neq y_i\}$, then this sample can be considered as a `regular' sample representing the class $y_i$. For such regular samples, we have a large  $y_i(\rvy_{-i}^\top\rvg_i)$, which results in a smaller CG(i). On the other hand, if a sample has a relatively small $\rvx_i^\top \rvx_j$ even with the samples of the same class $\{\rvx_j:y_j=y_i\}$, or the gap between $\sum_{j\in\{[n]: y_i= y_j\}} H_{ij}^\infty$ and $\sum_{j\in\{[n]: y_i\neq y_j\}} H_{ij}^\infty$ is small, then $y_i(\rvy_{-i}^\top\rvg_i)$ is small, which results in a larger CG(i). Thus, irregular samples will have a larger CG(i).
\item Clean label vs. noisy label: A sample with label noise tends to have a large CG-score since the order of two terms in subtraction at $y_i(\rvy_{-i}^\top\rvg_i)=\sum_{j\in\{[n]: y_i= y_j\}} H_{ij}^\infty-\sum_{j\in\{[n]: y_i\neq y_j\}} H_{ij}^\infty$ is effectively switched for label-noise samples. Thus, $y_i(\rvy_{-i}^\top\rvg_i)$ tend to be negative for a sample with label noise, while it is positive for clean-label samples. %Thus, the samples with label noise tend to have a larger CG-score.
\end{enumerate}


We empirically demonstrate the above two trends by a controlled experiment. 
Consider two 3000-dimensional Gaussian distributions with a fixed covariance matrix $0.25 I_{3000}$ and different means $(1,0,\dots 0)$ and $(-1,0,\dots,0)$, representing class +1 and -1, respectively.
We generate 1000 samples from each class. 
We first check whether the structural assumptions on $\rmH^\infty$ hold with this synthetic dataset. In Fig. \ref{fig:gaussian_heatgraph}, we observe that   $(\rmH^\infty)^{-1}_{n-1}$ can be well approximated by 2$I_{n-1}$, and thus the approximation for $\mathrm{CG}(i)$ in \eqref{eqn:vi_simp_approx} may hold well. 
We then examine the correlation between the CG-score and the sample value at the first dimension.
In Fig. \ref{fig:scatter_normal}, we can observe that instances near the decision boundary $x_1=0$ have higher CG-scores. This shows that irregular samples, e.g., samples near the boundary of the two classes, indeed have higher CG-scores. 
%To examine the CG-score  with label noise, 
We further modify the generated samples by randomly flipping the labels of 10\% samples and re-calculate the CG-scores of all the samples. As shown in Fig. \ref{fig:scatter_noise}, the samples with label noise tend to have higher CG-scores, agreeing with our intuition.
In Appendix \S\ref{app:sec:noise_atypical}, we further discuss discriminating mislabeled data and atypical (but useful) data by using CG-score, and also show high/low-scoring examples for public datasets including MNIST, FMNIST, CIFAR-10 and ImageNet in Appendix \S\ref{sec:app:visu}.
%Discriminating mislabeled data and atypical (but useful) data is a major challenge in data valuation, since both the mislabeled data and atypical data are irregular in the data distribution and tend to have high CG-scores. The same challenge has been observed with previous valuation scores such as forgetting score \citep{forgetting} and EL2N score \citep{EL2N}.

%However, we find that mislabeled data usually has a higher CG-score than atypical data, and this tendency gives us the possibility to separate mislabeled data from the rest of the clean data.


% that the CG-score can be used to detect samples with label noise even without training of a model.


%For synthetic data, we consider a mixture of two 3000-dimension Gaussian distributions. These two gaussian distributions have the same mean(0) and covariance matrix(identity matrix times 0.25) except for the mean value of the first dimension. We notice that the first dimension value becomes the criterion for determining the gaussian group due to the design of the distribution. We first check how many assumptions fit in experiments. As shown in Fig. \ref{fig:gaussian_heatgraph}, we observe that $(H^\infty)^{-1}_{n-1}$ is similar to 2$I_{n-1}$. This indicates that the approximations fit in this experiment. We also observe that mean of p is 0.0003, and mean of q is -0.0002. We then calculate the CG score using 1,000 generated samples per Gaussians and analyze the correlation between the high CG score sample and the first dimension value. As shown in Fig. \ref{fig:scatter_normal}, samples that are located by zero tend to have higher CG scores. This implies that the samples with high CG score are located  near its decision boundary.  We also calculate the CG score in 10\% noisy label case data and analyze the correlation between the high CG score sample and the first dimension value. As shown in Fig. \ref{fig:scatter_noise}, samples with label noise tend to have higher CG scores. This indicates that the CG score can be used to detect samples with label noise without training some models.




==> ICLR2023_CGscore (CameraReady)/section/4_exp_value.tex <==
\section{Data Valuation through Complexity Gap Score}\label{sec:exp_value}

%In this section, we show diverse applications of the CG-score in data valuation for real datasets.

%We next apply the CG-score to analyze public image datasets: FMNIST \citep{FMNIST_data} and CIFAR-10/100 \citep{CIFAR_data}.\footnote{Some examples of these public datasets, sorted by the CG-score, are displayed in Appendix \S\ref{sec:app:visu}.}
%We examine the samples with highest/lowest CG-scores by visualizing the examples in Section \ref{sec:data_vis}. 
%We first evaluate the CG-score in finding `important' examples by designing data pruning experiments in Section \ref{sec:data_pruning}.
%We also discuss the ability of the CG-score in detecting samples with label noise in Section  \ref{sec:noise_det}. 
%Before we move on to the experimental results, we first discuss how we calculated the CG-score for multi-label datasets. 
%We first examine the samples with highest/lowest CG-scores by visualizing the examples in Section \ref{sec:data_vis}. 
%In Section \ref{sec:noise_det}, we also plot 


%\paragraph{Calculation of CG-score for multi-label datasets}
%In defining the CG-score, we assumed the binary datasets $y\in\{\pm1\}$ with inputs having a fixed norm $\|\rvx\|_2=1$.To calculate the CG-score for multi-label ($k$-class) public datasets, we first normalize all the inputs to have $\|\rvx\|_2=1$. We then calculate the CG-score for examples of each class $j\in[k]$, by assuming that all the examples from class $j$ have label $+1$, and the rest of the examples from any other classes have label $-1$. Since the calculation of the CG-score requires the inversion of $n$-dimensional matrix $\rmH^\infty$ where $n$ is the number of total samples, to lower the complexity, we sub-sample the examples with class $-1$ so that the ratio between class +1 and class -1 is reduced from $1:(k-1)$ to $1:3$ for MNIST and FMINST and $1:4$ for CIFAR-10 and CIFAR-100. We repeat this process 10 times by randomly sampling examples of label $-1$ and then average out the calculated CG-score of each example from class $+1$. More details on the calculation of CG-score are available in Appendix \S\ref{sec: multi-class}.

%We explain how to calculate $CG$ score at the experiments. When we calculate the score, we normalize the input data $\rvx_{i}$ and generate the gram matrix $\rmH^\infty$ for every dataset. At 2-label dataset, we set the label of data as 1 and -1. At multi label dataset, we calculate $CG$ scores for each label data.
%We assign 1 to the label of corresponding label data and assign -1 to the label of other sampled data.
%We sample the data because calculation of $\rmH^\infty$ requires expensive memory and computational cost. As the calculation of the scores is stochastic, we calculate 10 times and average the score.
%More detailed information is explained at the appendix \ref{sec: multi-class}.


%\paragraph{Visualization of examples sorted by CG-score}%\label{sec:data_vis}
%\input{fig/visualize_exp/visualize_exp}
%\input{fig/visualize_exp/visualize_exp_CIFAR10} 
%In Fig \ref{fig:visualize_exp}, we show examples of MNIST (left) and FMNIST (right) images sorted by CG-score. The top/bottom three rows show the top-/bottom-ranked examples, respectively. We can observe that the examples with the lowest CG-scores are regular examples representing each class and they look similar to each other, while the examples with the highest scores are irregular and they look different among themselves, among which we can identify (possibly) mislabeled instances, marked with red rectangles. 

%In Fig \ref{fig:visualize_exp_CIFAR10}, we display ten top-ranked examples (top two rows) and ten bottom-ranked examples (bottom two rows) for three classes (Dog, frog and truck) of CIFAR-10 dataset. Similarly, low-scoring examples are regular ones, sharing similar features representing the class, while high-scoring examples are irregular ones. 
%We observe examples whose $CG$ scores are low look typical and clear. Otherwise, examples whose $CG$ scores are high look atypical, unclear, or noisy.
%we show ten top-ranked $CG$ score examples and ten bottom-ranked $CG$ score examples for three classes (Dog, frog and truck) in CIFAR10 dataset. Similarly, low score examples looks typical and high score examples looks atypical. 

% \subsection{Correlation with other scores}
% We calculate Spearman rank correlation between with $CG$ scores of CIFAR10 and CIFAR100 and previous scores, cscore, forgetting score, and EL2N score which is calculated at 10 epoch.

% \begin{table}
% \centering
% \caption{correlation - CIFAR10}
% \label{t1}
% \begin{tabular}{|c|c|c|c|}
% \noalign{\smallskip}\noalign{\smallskip}\hline
% - & cscore & forgetting & EL2N \\
% \hline
% $CG$ score & 0.557 & 0.432 & 0.365 \\
% \hline
% $CG'$ score & - & - & -  \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}
% \centering
% \caption{correlation - CIFAR100}
% \label{t1}
% \begin{tabular}{|c|c|c|c|}
% \noalign{\smallskip}\noalign{\smallskip}\hline
% - & cscore & forgetting & EL2N \\
% \hline
% $CG$ score & - & - & - \\
% \hline
% $CG'$ score & - & - & -  \\
% \hline
% \end{tabular}
% \end{table}

\subsection{Data pruning experiments}\label{sec:data_pruning}
\input{fig/pruning_exp/pruning_exp}
% \input{fig/new_pruning_exp/new_pruning_exp}
To evaluate the ability of the CG-score in identifying important examples, we design data pruning experiments, similar to those in \citet{shapley, EL2N}. 
We evaluate our score on three public datasets, FMNIST, CIFAR-10/100  and train ResNet networks \citep{resnet}, ResNet18  for FMNIST and CIFAR-10 and ResNet50 for CIFAR-100 dataset, respectively. As baseline methods for data valuation, we use three state-of-the-art scores, C-score \citep{cscore}, EL2N \citep{EL2N}, and Forgetting score \citep{forgetting}, all of which require training of models for computation. On the contrary, our score is a data-centric measure and independent on the model. More details on the baselines and experiments are summarized in Appendix \S\ref{sec:details}.
%More details on the baselines and experiments are summarized in Appendix \S\ref{sec:details}.
%\footnote{Our code is publicly available at \url{https://github.com/JJchy/CG_score}.}



%We conduct two directional experiments: 1) evaluating a model while training with a pruned dataset where different portions of low-scoring (regular) examples are removed to examine the generalization capability of the model with only high-scoring (irregular but possibly important) examples (the first row of Fig. \ref{fig:pruning_exp}); 2) the same experiment while pruning different portions of high-scoring examples to examine the generalization capability of the model with only low-scoring examples (the second row of \ref{fig:pruning_exp}). 
In Figure \ref{fig:pruning_exp}, the first row shows the test accuracy of the model trained with different subset sizes when low-scoring (regular) examples are removed first, while the second row shows the similar result but when high-scoring (irregular) examples are removed first. 
We report the mean of the result after {five} independent runs, and the shaded regions indicate the standard deviation.
The gray line (full dataset) represents the results when all data is used, while the red curve (random) represents the results when examples are randomly removed.
We can observe that when removing low-scoring examples first, networks maintain the test accuracy up to significant removing portions, i.e., 40\% for CIFAR-10 and 20\% for CIFAR-100 with less than 1\% test accuracy drop. Our CG-score, which does not require any training of a model, can achieve competitive performances as the other baseline methods and it also significantly outperforms the random baseline. When removing the high-scoring examples first, the test accuracy drops most rapidly for the CG-score curve, implying  that examples with the high CG-score are essential part of the data governing the generalization of the model. 

We show the effectiveness of CG-score in more complicated models and also in fine-tuning by reporting the data pruning experiments at  DenseNetBC-100 \citep{densenet} and  Vision Transformer (ViT) \citep{ViT} in Appendix \S\ref{sec:model variant}. We also compare CG-score with two more baselines, TracIn \citep{tracin} and CRAIG \citep{CRAIG}, in Appendix \S\ref{sec:additional baselines}.
%\change{In addition, we conduct several additional experiments and provide these at appendix. At first, to check that ``model invariant CG-score" works well at various model, we conduct data pruning experiments at additional networks, DenseNet and ViT, and provide the results at Appendix \S\ref{sec:model variant}. %Next, we propose CG-score also has validity at relatively complex dataset, the ImageNet, and provide result at Appendix \S\ref{sec:app:visu}. 
%Furthermore, we provide results of additional baselines at Appendix \S\ref{sec:additional baselines}.}
%We conduct a data pruning experiment to check how well our score empirically evaluates data. In the data pruning experiment, we remove the high-scoring or low-scoring data after sorting the dataset with the score and then check the final performance of each training. Before explaining the experimental results, we describe the details of the experiment.

%\paragraph{Experiment details} 
%We also use FMNIST, CIFAR10/CIFAR100 as the training dataset. We evaluate our method on widely-studied ResNet networks(\cite{resnet}) to train each dataset: ResNet18 (FMNIST, CIFAR10), ResNet50 (CIFAR100).
%C-score(\cite{cscore}), EL2N(\cite{EL2N}), and Forgetting(\cite{forgetting}) score is used as other scores to be compared, and each score is independently measured at different time. Unlike other scores, C-score's trend is the opposite, so the trend was adjusted by multiplying by -1 in the experiment. We obtain three independent training results for each experiment and represent its mean and one standard deviation above and below the mean by shading the area in the graphs. 
%Configurations, hyperparameters, and other details are available in Appendix \S\ref{sec:details}. 


%In the first row of the figure \ref{fig:pruning_exp}, we observe that the CG score, similar to other scores, maintains performance even when low score data is pruned to some extent different from the random case. This indicates that each score reflects the value of the data, so performance does not decrease even if data with a low value is excluded. Similarly, in the second row of the figure \ref{fig:pruning_exp}, we observe a sharp performance drop when high score data are pruned except for random case, which means that the data with a high value is essential for learning performance. 

%From the experiment, we observe that the CG score has competitive data valuation performance compared to other state-of-the-art scores in several datasets. We note that the CG score is only dependent on the dataset itself, which indicates that a certain extent of data valuation is already possible with only the dataset, regardless of any model or how much the model is trained.




\subsection{Detecting label noise}\label{sec:noise_det}

\input{fig/noise_exp/noise_detection}
In Section \ref{sec:geo_analysis}, we analyzed the CG-score and showed that the examples with label noise tend to have higher CG-score.
We next empirically investigate the ability of the CG-score in detecting label noise by artificially corrupting 20\% of instances in FMNIST and CIFAR-100 with random label noise.
We first examine the distribution of the CG-scores for each dataset after the corruption in Figure \ref{fig:noise_dist1}.
We can observe that for both datasets, the examples with corrupted labels (orange) tend to have higher CG-scores than those with clean labels (blue).
For a relatively simpler dataset, FMNIST (left), the CG-score histograms can be more clearly separable between the clean and noisy groups, compared to a more complex dataset, CIFAR-100 (right).
%We can observe that for a relatively simpler dataset such as FMNIST, the examples with corrupted labels have CG-scores much higher than those with the clean labels, so that the CG-score histograms can be separable between the clean and noisy groups. On the other hand, for more complex datasets such as CIFAR-100, the examples with label noise tend to have higher CG-score, but the histograms for clean labels and noise labels cannot be well separable. 
With this observation, we can anticipate that the CG-score can have a better detectability of label noise for relatively simpler datasets.

We evaluate the noise detectability of the CG-score by checking a varying portion of the examples sorted by the CG-score (highest first) in Fig. \ref{fig:noise_det1}. The curves indicate the fraction of noisy examples included in the examined subset. 
We compare our score with two other scores, Forgetting score and EL2N, as well as a random baseline and the oracle. 
We can observe that the CG-score achieves the best performance, near that of the oracle, for FMINST, and competitive performances for CIFAR-100. In the plot, we also compare the performance of the CG-score with that of `Partial CG-score,' which is a new score defined by a sub-term of the CG-score. In the CG-score in \eqref{eqn:vi_simp}, we have three terms, but only the second term $2y_i( \rvy_{-i}^\top\rvh_i )$ uses the label information of the data $(\rvx_i,y_i)$. Thus, we examined the ability of this term only, defined as the `Partial CG-score', in detecting the label noise, and found that the CG-score and partial CG-score have similar performances in detecting label noise, which implies that the label-noise detectability of the CG-score mainly comes from the term $2y_i( \rvy_{-i}^\top\rvh_i )$. 
More experiments with higher noise rate are reported in Appendix \S\ref{sec:score_dist}.
%\change{Furthermore, inspired by that the feature of data has better representation than data itself, we develop the feature-space CG-score, which is calculated by feature of data instead of data input. We check that the new score has a remarkable performance by conducting data pruning experiment and noise detection experiment and provide the result at Appendix \S\ref{sec:feature_CG}.}

% \beq\label{eqn:vi_simp}
%v(i)= d_i^{-1}(\rvy_{-i}^\top\rvh_i)^2+2y_i( \rvy_{-i}^\top\rvh_i )+y_i^2 d_i=\left({(\rvy_{-i}^\top\rvh_i)}/{\sqrt{d_i}}+y_i\sqrt{d_i}\right)^2.
%\eeq
%We corrupt 20\% of datasets, then calculate $CG$ scores, forgetting scores, and EL2N scores of the noisy datasets. Then we check how many noisy data are detected among data whose scores are high.
%In addition, we introduce '$Partial CG$ scores', which removes terms those are not related with label information from $CG$ score.
%Note that $CG(i)=d_i^{-1}(\rvy_{-i}^\top\rvh_i)^2+2y_i( \rvh_i^\top \rvy_{-i})+y_i^2 d_i$, but $d_i^{-1}(\rvy_{-i}^\top\rvh_i)^2$ and $y_i^2 d_i$ are terms without information of label $y_i$ (${y_i}^2 = 1$).
%At noise detection, we propose the $Partial\, CG$ scores $2y_i( \rvh_i^\top \rvy_{-i})$ as a new score, and check this new score has better noise detectability than $CG$ scores.

%Experimental results show that the $Partial\, CG$ scores and the $CG$ scores could detect noise. 
%The noise detectability of $Partial\, CG$ scores and $CG$ scores were superior to the other scores at noisy FMNIST dataset.
%However, as the dataset becomes complex, $CG$ scores distributions of the clean and noisy data becomes 
%hard to distinguish.
%As a result, noise detectability of two scores are weaken at complex dataset.

%We analyze the reason that 
%CG score가 데이터� 복잡해지면 잘 안되는 이유 : CG score가 2-layer overparameterized net에서 유도되는 값인데, 2-layer로 복잡한 데이터의 특성을 나타내기에는 한계가 있기 때문에
%$CG$ scores were derived 2-layer overparameterized network.

%Noisy data has higher score than clean data, and it is easier to distinguish noisy data for simple dataset. 
%Histogram of scores shows the separability of the dataset. 

% \input{fig/noise_exp/FMNIST_noise_exp}
% \input{fig/noise_exp/CIFAR10_noise_exp}

==> ICLR2023_CGscore (CameraReady)/section/5_exp_dyn.tex <==
\section{Complexity-Gap Score and Deep Learning Phenomena}\label{sec:exp_dyn}

We next demonstrate that the CG-score can capture `learning difficulty' of data instances.% for CIFAR-10 dataset trained in ResNet18.
%, by comparing the loss and accuracy of different sub-groups of instances, sorted by the CG-score, throughout the training in Section  \ref{sec:learning_diff} and by analyzing the evolution velocity of Neural Tangent Kernel (NTK) submatrices defined by the sub-groups of the data sorted by the CG-score in \ref{sec:NTK}.

% the training dynamics of individual instances--the behavior of a network on individual instances during training. 
%In Section \ref{sec:learning_diff}, we show that the CG-score can reflect the learning difficulty of a sample on the model, by comparing the loss and accuracy of different sub-groups of instances, divided by the CG-score. We find that the high-scoring data instances are learned much slowly, compared to the low-scoring groups. 
%In Section \ref{sec:NTK}, we further examine how each sub-group of data instances, divided by the CG-score, differently contributes in the optimization of the neural network by measuring and comparing the evolution velocity of Neural Tangent Kernel (NTK) submatrices, defined by the sub-groups of the data. We find that the NTK submatrices of high-scoring groups change by a larger amount throughout the training compared to those of low-scoring groups. This shows that the instances with high CG-score are the ones deriving the optimization of the model.  

\input{fig/dynamic_exp/dynamic_exp}
\subsection{Complexity gap score captures learning difficulty}\label{sec:learning_diff}

It has been widely observed that there exists an order of instances in which a model learns to classify the data correctly and this order is robust within model types  \citep{curricula}. Many previous scoring functions use this type of observation and define the `difficulty' of a given instance based on the speed at which the model's prediction converges  \citep{forgetting, carto}. 
Our data-centric CG-score is originally defined based on the gap in the generalization error bounds as in \eqref{def:vi}, but it also reflects the convergence speed of the instance, as analyzed in \eqref{eqn:acc}.
We empirically demonstrate this relation by analyzing the training dynamics of CIFAR-10 dataset trained in ResNet18 network. We first sort the data instances in ascending order using the CG-score, and divide the data into 10 equal-sized subgroups. We then measure the mean of loss and training accuracy for the 10 subgroups as training progresses. Fig. \ref{fig:dynamic_loss} and Fig. \ref{fig:dynamic_acc} show the mean of loss and the training accuracy throughout the training for the 10 subgroups, respectively, where the blue color represents the low-scoring groups and the red color represents the high-scoring groups. We can observe that the mean loss and accuracy converge faster for low-scoring groups, while it takes longer to converge for high-scoring groups. This indicates that the CG-score is highly correlated with the `difficulty' of an example measured by the learning speed at a model. 

%In this section, we explain that our CG score captures the learning difficulty of each data in the training set. \cite{curricula}, \cite{cscore} paper mention that the more complex the data, the slower the learning speed of the data. To show this better, we sorted the data in ascending order based on the CG score and divided the CIFAR-10 data into ten equal groups. After that, we train the ResNet18 model, typically using all CIFAR-10 data, and measure each group's training dynamics(mean of loss and group accuracy).
%Figure \ref{fig:dynamic_loss} and \ref{fig:dynamic_acc} shows how the loss mean and accuracy change for each group among each epoch. Each line's color varies from blue to red according to the size of the CG score. 
%From the figure, we observe that the loss and accuracy of groups with low CG scores converge within a few epochs, and the loss and accuracy of groups with high CG scores require more epochs to converge.
%This indicates that the CG score is highly correlated with the example difficulty in the dataset.

\subsection{Data samples driving movement of neurons}\label{sec:NTK}

We next investigate the relation between the CG-score and the evolution velocity of the data-dependent Neural Tangent Kernel (NTK) \citep{fort2020kernel_velocity}.
NTK has been widely used to approximate the evolution of an infinite-width deep learning model via linearization around initial weights, when the network is trained by gradient descent with a sufficiently small learning rate \citep{jacot2018neural}.  The main idea is that in the limit of an infinite width, the network parameters do not move very far from its initialization throughout the training, so that the learning process can be approximated by a linear process along the tangent space to the manifold of the model's function class at the initialization \citep{lee2019wide}. However, as observed in \citet{fort2020kernel_velocity}, for a finite-width network, the tangent kernel is not constant but it rather rapidly changes over time, especially at the beginning of the training. 
To quantify this change,  \citet{fort2020kernel_velocity} addressed the data-dependent Kernel Gram matrix, which is the Gram matrix of the logit Jacobian, and defined the Kernel velocity as the cosine distance between two NTK Gram matrices before and after one epoch of training. 
In \cite{EL2N}, the Kernel velocity was used to evaluate the subgroups of data instances to figure out the subgroup driving the learning and the change in the NTK feature space. We conduct similar experiments for subgroups of data, divided according to our CG-score.
Fig. \ref{fig:dynamic_ntkv} shows the Kernel velocities for 10 different subgroups of CIFAR-10 data trained in ResNet18.  Each group is composed of 125 consecutive instances from each level, where the level is defined by dividing the full dataset, sorted in ascending order by the CG-score, into 10 groups. The higher level (red) is composed of instances having higher CG-scores, while the lower level (blue) is composed of instances having lower CG-scores. We can observe that the samples with high CG-score (red) maintains higher Kernel velocity throughout the training, which means that NTK Gram matrix evolves by a larger amount for the samples of high CG-score. Thus, we can hypothesize that the instances with high CG-score are `difficult' examples the network may struggle to optimize and try to fit throughout the training. 

%We next explain that our CG scores are associated with samples that frequently change model parameters during training. In equation \ref{eqn:acc}, We show that the accumulated difference between a label and current network output would be correlated with the CG-score. This means that a sample with a large CG-score is correlated with the sample with a large difference between a label and network output at a specific epoch, which means that the network is constantly struggling with these samples. As the network continues to adapt to a dataset, the gradient of the complex examples changes greatly in epochs.

%We empirically show this tendency to train ResNet18 network on the CIFAR-10 dataset. We sample ten groups which consist of consecutive 125 subsets and equally spaced apart based on CG score and calculate the kernel velocity(\cite{fort2020kernel_velocity}, \cite{EL2N}) of these groups at each epoch. The kernel velocity is a value that measures the change of data-dependent NTK in a group. If this value is large, it means that the gradient in the groupp changes greatly in epochs. The details of kernel velocity are available in Appendix \S\ref{sec:kernel_velocity}. From the figure \ref{fig:dynamic_ntkv}, we observe that the kernel velocity is higher in the group with a higher CG score and decreases overall as the epoch pass. 


% \subsection{Data augmentation using complexity gap score}

==> ICLR2023_CGscore (CameraReady)/section/6_discussion.tex <==
\section{Discussion}\label{sec:dis}

We proposed the CG-score, a data-centric valuation score, to quantify the effect of individual data instances in optimization and generalization of overparameterized two-layer neural networks trained by gradient descent. We theoretically and empirically demonstrated that the CG-score can identify `irregular' instances within each class, and can be used as a score to select instances essential for generalization of a model or in filtering instances with label noise. We also showed the close relation between the CG-score and learning difficulty of instances by analyzing training dynamics. Interesting open problems related to the CG-score include 1) providing theoretical justification of the score for more general deep neural networks and 2) improving the score by modifying the definition in terms of `features' of data instances. In Appendix \S\ref{sec:feature_CG}, we provide further discussion for `feature-space CG-score' and report experimental results, demonstrating the effectiveness of the score.

%\change{
%CG-score has an huge advantage since we do not need to find an appropriate model with parameters and train it, However, when domain shift exists, this algorithm can not valuate how much the target data is valuable to express testset distribution.
%Huge number of data in a class or multi label dataset require large matrix, which causes expensive computational cost. Stochastic method enables us to reduce the cost, however, still the algorithm was more expensive than previous method in some cases.}


%We propose CG-scores which valuates the data without a train of a neural network, otherwise previous researches on data valuation are relies on the train. CG-score, which is defined as gap of generalization error bound when the target data is removed, has two theoretical meanings. - In high dimensional Gaussian model, data located close to the decision boundary has high CG-score. It is because gram matrix can be approximated as constant times of an identity matrix, the score is proportional to sum of angles between different label data and inversely proportional to sum of same label data. Therefore, data whose CG-scores are high are helpful to find decision boundary.

%In neural network, CG-score is equal with contribution to the total network variation. 

%CG scores have clear pros and cons,
%pros : Algorithm to calculate the score is simple and required computational complexity is low.
%cons : Other scores which utilize a train of a complex neural network has better performance.

%Since CG-scores are derived from 2-layer overparameterized network, performances of the scores become poorer for complex datasets which can not be expressed well by the 2-layer network.

%There are some remained works to do.
%Theoretical meanings of the CG-scores can not be applied at multi-label case.
%Because the score does not utilize a train of neural network, it clearly has a limitation.
%Although, it needs to find a method to achieve higher performances as data valuation.
%Normalization of the data loose information. Algorithm without normalization of the data is .

%CG-scores give us a message : Information of angles among the data possess potential to express


==> ICLR2023_CGscore (CameraReady)/table/computational_cost.tex <==
\begin{table}[tbh]
\centering
\caption{Time cost(seconds) to compute scores of the dataset.}
\label{tab:computational_cost}
\begin{tabular}{{c|ccc}}
\toprule
\color{blue}
& FMNIST & CIFAR-10 & CIFAR-100 
\\
\midrule
CG-score 1:1 & 1063 & 608  & 37.9 \\
CG-score 1:2 & 2610 & 1497 & 40.3 \\
CG-score 1:3 & 4834 & 2773 & 49.0 \\
CG-score 1:4 & -    & 4388 & 61.1  \\
Forgetting & 1879   & 3322 & 6675 \\
EL2N & 370 & 323 & 662 \\
TracIn & 1856 & 3425 & 8400 \\
CRAIG & 3023 & 5263 & 10472 \\
\midrule
GPU & \multicolumn{3}{c}{Nvidia A100 40GB} \\
\bottomrule
\end{tabular}
%\vspace{-1em}
\end{table}

==> ICLR2023_CGscore (CameraReady)/table/detailed_parameter.tex <==
\begin{table}[tb!]
\centering
\caption{Details for the experiments used in the training of the dataset.}
\label{tab:detail}
\begin{tabular}{m{0.3\textwidth} | m{0.2\textwidth} m{0.2\textwidth} m{0.2\textwidth}}
\toprule
& FMNIST & CIFAR10 & CIFAR100 
\\
\midrule
Architecture & ResNet18 & ResNet18 & ResNet50 \\
Batch size & 128 & 128 & 128 \\
Epochs & 100 & 200 & 200 \\
Initial Learning Rate & 0.02 & 0.05 & 0.1 \\
Weight decay & 5e-4 & 5e-4 & 5e-4 \\
Optimizer & \multicolumn{3}{l}{SGD with momentum 0.9} \\
Learning Rate Scheduler & \multicolumn{3}{l}{Cosine annealing schedule \citep{loshchilov2017cosineannealing}} \\
\midrule
Data Augmentation & \multicolumn{3}{l}{\begin{tabular}[l]{@{}l@{}}Normalize by dataset's mean, variance \\ Random Zero Padded Cropping (4 pixels on all sides) \\ Random left-right flipping (probability 0.5)\end{tabular}} \\
\bottomrule
\end{tabular}
%\vspace{-1em}
\end{table}

==> ICLR2023_CGscore (CameraReady)/table/rank_corr.tex <==
\begin{table}[tb]
\centering
\caption{Spearman's rank correlation between CG-score (CG'-score) and other data valuation scores. }
\label{tab:rank_corr}
\vspace{0.2em} \small{ 
\begin{tabular}{c|ccc| ccc}
\toprule
\multirow{2}{*}{Datasets} & \multicolumn{3}{c|}{Correlation btwn. CG-score and} &\multicolumn{3}{c}{Correlation btwn. CG'-score and}
\\
 &C-score  & Forgetting & EL2N &C-score  & Forgetting & EL2N  \\
\midrule
CIFAR-10 &0.557 & 0.432 & 0.365 & 0.115 & 0.110 & 0.136\\
CIFAR-100 & 0.529 & 0.289 & 0.356& 0.243&0.090 &0.177 \\
\bottomrule
\end{tabular}}
%\vspace{-1em}
\end{table}

==> fig/visualize_exp/CIFAR_mean_std.tex <==
\begin{figure*}[!tb]
\centering
	{\includegraphics[width=0.47\linewidth]{fig/visualize_exp/CIFAR100_means_std.png}}
	\label{fig:CIFAR100_means_std}
\end{figure*}

==> fig/visualize_exp/Imagenet.tex <==
\begin{figure*}[!htb] 
\centering
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/Imagenet_figure.png}}
    \\
    \subfloat[Examples and histograms of four classes in Imagenet\label{fig:imagenet_means_four}]
	{\includegraphics[width=1\linewidth]{fig/visualize_exp/Imagenet_hist.png}}
    % \hfill
    % \subfloat[CIFAR100-Flatfish \label{fig:Frog}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_bottle_hist.png}}
    % \hfill
    % \subfloat[CIFAR10-Orange \label{fig:Truck}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_orange_hist.png}}
    % \subfloat[CIFAR10-plain \label{fig:Truck}]{\includegraphics[width=0.24\linewidth]{fig/visualize_exp/CIFAR100_class_plain_hist.png}}
    
    \caption{\change{Sample analysis for Imagenet in terms of the CG-score. Figure shows 4 top-ranked examples (top rows) and 4 bottom ranked examples (bottom rows) for Cypripedium, Oxcart, Orange, and Horn classes of Imagenet dataset. Histograms show distributions of the CG-scores for each class.}}
\label{fig:visualize_Imagenet}
\end{figure*}

==> fig/visualize_exp/visualize_exp_CIFAR10.tex <==
\begin{figure*}[!tb] \label{fig:CIFAR10_image_hist_}
\centering

	{\includegraphics[width=1\linewidth]{fig/visualize_exp/CIFAR10_image_.png}}
    \\
    %{\includegraphics[width=1\linewidth]{fig/visualize_exp/CIFAR10_image_hist_.png}}
    \caption{Top-ranked examples (top two rows) and bottom ranked examples(bottom two rows) for four classes of CIFAR-10 dataset.}
    \label{fig:visualize_exp_CIFAR10}
\end{figure*}
